Graphs are everywhere -- Psst! In Music Recommendation too

In recent years, graphs have gained prominence across various domains, especially in recommendation systems. Within the realm of music recommendation, graphs play a crucial role in enhancing genre-based recommendations by integrating Mel-Frequency Cepstral Coefficients (MFCC) with advanced graph embeddings. This study explores the efficacy of Graph Convolutional Networks (GCN), GraphSAGE, and Graph Transformer (GT) models in learning embeddings that effectively capture intricate relationships between music items and genres represented within graph structures. Through comprehensive empirical evaluations on diverse real-world music datasets, our findings consistently demonstrate that these graph-based approaches outperform traditional methods that rely solely on MFCC features or collaborative filtering techniques. Specifically, the graph-enhanced models achieve notably higher accuracy in predicting genre-specific preferences and offering relevant music suggestions to users. These results underscore the effectiveness of utilizing graph embeddings to enrich feature representations and exploit latent associations within music data, thereby illustrating their potential to advance the capabilities of personalized and context-aware music recommendation systems. Keywords: graphs, recommendation systems, neural networks, MFCC

==> z_extra.tex <==
\begin{table*}[t]
\centering
\caption{Accuracy scores by genre and person}
\label{accuracy_scores}
\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrrrrrr}
\toprule
& \texttt{Person1} & \texttt{Person2} & \texttt{Person3} & \texttt{Person4} & \texttt{Person5} & \texttt{Person6} & \texttt{Person7} & \texttt{Person8} & \texttt{Person9} & \texttt{Person10} \\
\midrule
Electronic & 0.55 & 0.72 & 0.60 & 0.54 & 0.42 & 0.65 & 0.44 & 0.89 & 0.96 & 0.38 \\
Experimental & 0.54 & 0.53 & 0.57 & 0.93 & 0.07 & 0.09 & 0.02 & 0.83 & 0.78 & 0.87 \\
Folk & 0.98 & 0.80 & 0.90 & 0.78 & 0.75 & 0.64 & 0.94 & 0.94 & 0.72 & 0.81 \\
Hip-Hop & 0.58 & 0.63 & 0.77 & 0.77 & 0.76 & 0.81 & 0.64 & 0.67 & 0.67 & 0.81 \\
Instrumental & 0.75 & 0.85 & 0.87 & 0.82 & 0.71 & 0.69 & 0.76 & 0.57 & 0.65 & 0.71 \\
International & 0.57 & 0.44 & 0.99 & 0.10 & 0.21 & 0.16 & 0.65 & 0.25 & 0.47 & 0.24 \\
Pop & 0.66 & 0.69 & 0.72 & 0.80 & 0.75 & 0.67 & 0.81 & 0.66 & 0.68 & 0.73 \\
Rock & 0.85 & 0.89 & 0.76 & 0.90 & 0.86 & 0.75 & 0.91 & 0.93 & 0.65 & 0.81 \\
\bottomrule
\end{tabular}
}
\end{table*}

\subsection{Subjective Results}
A subjective study was conducted to gauge the sentiment of the humans and help in comparing the results from the previous section. The study was conducted as follows. Each person was made to hear 10 songs of each genre and was subsequently given the task of categorizing each song. Although the results have high variability in them, certain patterns were clearly observable. The following table summarizes the categorization of genres. It is seen that Pop, Rock, Folk, and Hip-Hop genres were easy for the user to distinguish while other genres posed some problems. Particularly a low score in differentiating Electronic from Experimental is a recurring pattern. Instrumental and International genres are pretty have produced unpredictable results and it is worth noting this pattern. One should also keep in mind that the chosen song was randomly cut into 5-second frames hence this result. Possibly a longer version would have rendered better numbers. This again goes on to show that algorithms can effectively work even with a 5-second window of random choice. 
